YoloTag: Vision-based Robust UAV Navigation with Fiducial Markers

By harnessing fiducial markers as visual landmarks in the environment, Unmanned Aerial Vehicles (UAVs) can rapidly build precise maps and navigate spaces safely and efficiently, unlocking their potential for fluent collaboration and coexistence with humans. Existing fiducial marker methods rely on handcrafted feature extraction, which sacrifices accuracy. On the other hand, deep learning pipelines for marker detection fail to meet real-time runtime constraints crucial for navigation applications. In this work, we propose YoloTag -a real-time fiducial marker-based localization system. YoloTag uses a lightweight YOLO v8 object detector to accurately detect fiducial markers in images while meeting the runtime constraints needed for navigation. The detected markers are then used by an efficient perspective-n-point algorithm to estimate UAV states. However, this localization system introduces noise, causing instability in trajectory tracking. To suppress noise, we design a higher-order Butterworth filter that effectively eliminates noise through frequency domain analysis. We evaluate our algorithm through real-robot experiments in an indoor environment, comparing the trajectory tracking performance of our method against other approaches in terms of several distance metrics.

==> sect/experiment.tex <==
\subsection{Setup}
% All the experiments were tested on a desktop computer with Intel(R) Core(TM) i7-10700 CPU @ 2.90GHz with an NVIDIA Quadro P2200 GPU which have GPU memory of 5 GB, and 32 GB of memory. The system operated on Ubuntu 20.04 LTS with ROS Noetic integration.
% \subsection{Experimental setup}
The experiments were conducted on a desktop computer equipped with an Intel(R) Core(TM) i7-10700 CPU @ 2.90GHz and an NVIDIA Quadro P2200 GPU, boasting a GPU memory of 5 GB, along with 32 GB of RAM. The system ran on Ubuntu 20.04 LTS integrated with ROS Noetic.
For capturing ground truth trajectories, a VICON Motion Capture System was employed, which operated on a separate computer with a AMD 7900X processor, 64 GB of memory with an NVIDIA GTX 4090 graphics card. Data transfer between the VICON system and the main desktop computer was facilitated through a ROS bridge.
% The VICON system comprised eight cameras for 0.1mm precise localization. 
% The motion capture system is set up in a work envelope of 6.10 meter long and 5.98 meter wide, providing ample space for the robot's action. 
% Eight Apriltag (36h11 family) landmarks with tag ids $1-8$, each measuring 0.2 meter in size, were separately positioned within the environment for localization using tag detections from the UAV camera. 
Eight Apriltag markers from the 36h11 family were positioned on the wall to sever as landmarks within our target environment. The markers ranged sequentially from 1 to 8, with each marker measuring 0.2 meters in size.
For all experiments evaluating the performance of YoloTag, a Parrot Bebop2 quadrotor-UAV was employed. The Bebop2 established a wireless connection to a desktop computer via the bebop2 autonomy ROS wrapper. Images captured by the onboard camera underwent processing to estimate the Bebop2's state. Subsequently, a PID controller facilitated real-time control of the Bebop2's motion through commands issued from the desktop computer.

% A Parrot Bebop2 quadrotor-UAV (Bebop2) was used in all experiments to evaluate the performance of YoloTag. Bebop2 was connected to a desktop using a wireless connection through the bebop2 autonomy ROS wrapper. Onboard camera images were processed to localize the Bebop2 and a PID controller was used to control the Bebop2 in real-time speed using the desktop computer.
 % The unmanned aerial vehicle (UAV) used in the experiment is a Bebop2 quadcopter from Parrot, controlled through a ROS wrapper for the Bebop2. This setup allows the UAV to accurately capture the markers from any distance within the designated work envelope using its onboard camera, enhancing the overall precision and reliability of the localization process.


% \subsection{Evaluating YOLO v8 based Marker Detection}
% Video data containing visual fiducial markers was collected via an unmanned aerial vehicle (UAV), a Parrot Bebop2 Drone equipped with a 14-megapixel F2.3 fish-eye camera, capturing images at 30 fps with a resolution of 856x480 pixels, and stored as a rosbag. 

% Training images were collected by flying our Bebop2 in a closed indoor environment as shown in Fig.~\ref{fig:vicon_setup} and Fig.~\ref{fig:bebop2_with_marker}. Multiple experiments were conducted to generate dataset by capturing on-board camera images at 30 fps with a resolution of 856x480 pixels using rosbag formats.

\subsection{Dataset Generation}
% To obtain training, validation, and testing images, the Bebop2 was flown within a closed indoor environment, as depicted in Figs. ~\ref{fig:vicon_setup} and ~\ref{fig:bebop2_with_marker}. 
% The environment was a $6.10\text{ m} \times 5.85\text{ m} \times 2.44\text{ m}$ where Eight Vicon cameras were mounted $0.30$ m from the ceiling to capture the full motion of the UAV as shown in Fig.~\ref{fig:vicon_setup}. Eight Fiducial Landmarks were statically pasted on the wall. Each landmark had a unique ID that allows the UAV to differentiate them when detected in the camera's field of view, enabling the UAV to estimate its state from the tags as shown in Fig.~\ref{fig:bebop2_with_marker}. 
% Multiple experiments were conducted to generate the dataset, capturing onboard camera images at $30$ frames per second (FPS) with a resolution of $856 \times 480$ pixels. 
% Vicon markers were used to capture the ground truth trajectories for all experiments. 
% Training image sequences and ground truth trajectories were recorded in rosbag format.
To obtain training, validation, and testing images, the Bebop2 was flown within a closed indoor environment measuring $6.10$ m × $5.85$ m × $2.44$ m, as shown in Figs.~\ref{fig:vicon_setup} and ~\ref{fig:bebop2_with_marker}.  Eight Vicon cameras were mounted on a speed rail to capture the full motion of the UAV, as depicted in Figs.~\ref{fig:vicon_setup}. Eight fiducial markers, each bearing a unique id, were affixed in static positions on the wall. The center of each marker was positioned precisely 0.724 meters from the ground. Furthermore, the distance separating any two neighboring markers measured 0.58 meters. This allowed the UAV to differentiate between the landmarks when detected in the camera's field of view, enabling the estimation of its state from the tags, as illustrated in Fig.~\ref{fig:bebop2_with_marker}.
Multiple experiments were conducted to generate the dataset, capturing onboard camera images at $30$ frames per second (FPS) with a resolution of $856 \times 480$ pixels. Vicon markers were used to capture the ground truth trajectories for all experiments. The training image sequences and ground truth trajectories were recorded in rosbag format.

\begin{figure}[htb]
    \centering
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=0.8\linewidth]{figs/vicon_setup.png}
        \caption{}
        \label{fig:vicon_setup}
    \end{subfigure}
    % \vspace{7pt}
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[width=\linewidth,height=0.8\linewidth]{figs/bebop2_flight.pdf}
        \caption{}
        \label{fig:bebop2_with_marker}
    \end{subfigure}
    \caption{The dataset was generated by flying a Bebop2 within a closed environment measuring $6.10$ m × $5.85$ m × $2.44$ m. A Vicon motion capture system (Fig.~\ref{fig:vicon_setup})  was employed to capture the UAV's motion, while the onboard camera was used to capture fiducial landmarks (Fig.~\ref{fig:bebop2_with_marker}), enabling the generation of ground truth data.}
    \vspace{-15pt}

    % \caption{The environment was a 
    % $6.10\text{ m} \times 5.85\text{ m} \times 2.44\text{ m}$ where Eight Vicon cameras were mounted $0.30$ m from the ceiling to capture the full motion of the UAV as shown in Fig.~\ref{fig:vicon_setup}. Eight Fiducial Landmarks were statically pasted on the wall. Each landmark had a unique ID that allows the UAV to differentiate them when detected in the camera's field of view, enabling the UAV to estimate its state from the tags as shown in Fig.~\ref{fig:bebop2_with_marker}. The Vicon System generates ground truth trajectories that serve as benchmarks for evaluating the trajectories produced by other methods.}
\end{figure}

\subsection{Training and Evaluation of YOLO v8}

For training the YOLO v8 model, we utilized $9,128$ images as the training set, $5,016$ images for the validation set, and $3,148$ images for the test set.
Initial automated annotation of the fiducial markers was performed using the Apriltag detection algorithm. However, as Apriltag could not accurately annotate all markers in every image, manual annotation was carried out utilizing an online tool to draw bounding boxes around the missing requisite visual markers.
To achieve real-time performance, we trained a lightweight YOLO V8 model that had been pre-trained on the MS-COCO dataset. The YOLO V8 model underwent training for $10$ epochs, enabling it to classify and localize fiducial markers within image frames by generating bounding box predictions.

% However, this approach exhibited insufficient reliability in detecting all necessary markers. To enhance detection accuracy, manual annotation was conducted utilizing an online tool to annotate bounding boxes around missing requisite visual markers. This produced a dataset mapping images to ground truth bounding box coordinates of salient landmarks. We have used 9128 images as the train dataset, 5016 images for the validation dataset, and 3148 images for the test dataset for training YOLOv8. We have used apriltag (3611h) markers only in the setup, and we had 8 markers with a size of 0.2m in the setup.

% Leveraging this manually annotated dataset in conjunction with the Apriltag detection dataset, we trained a lightweight Yolo V8 object detection model to perform real-time visual identification and localization in the pixel domain. YOLOv8 was trained for 10 epochs to optimize performance. It is noteworthy that our system is not constrained solely to Apriltags; it possesses the capability to detect other checkerboard markers as well, thereby enhancing its versatility and applicability in various scenarios.

Fig.~\ref{fig:subfig1} illustrates a recall-confidence curve that demonstrates the performance of the YOLO V8 model on the fiducial marker detection task. It is evident from this figure that the trained YOLO V8 model exhibited robust performance in detecting fiducial markers under varying conditions, such as image quality degradation and motion blur while following a desired trajectory.
Unlike the recall-confidence curve, which focuses solely on the recall metric, the F1-confidence curve, shown in Fig.~\ref{fig:subfig4}, takes into account both precision and recall, combining them into a single metric known as the F1 score. The F1 score is the harmonic mean of precision and recall, providing a balanced measure of the model's performance by considering both false positives and false negatives. As evident from Fig.~\ref{fig:subfig4}, our trained YOLO V8 model achieves a high F1 score, indicating that the model strikes a good balance between minimizing false positives and minimizing false negatives.

\begin{figure}[htb]
\centering
    \vspace{10pt}
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[trim=1cm 0cm 7cm 0cm, clip, width=\linewidth]{figs/R_curve.png}
        \caption{}
        \label{fig:subfig1}
    \end{subfigure}~
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[trim=1cm 0cm 7cm 0cm, clip, width=\linewidth]{figs/F1_curve.png}
        \caption{}
        \label{fig:subfig4}
    \end{subfigure}
\caption{ 
In Fig.~\ref{fig:subfig1} the blue line represents the average recall score across all markers while the other lines represent individual markers. 
As the confidence approaches 1.0, the recall sharply declined to 0.1, resulting in a 90 percent miss of true positives.
Similarly, Fig.~\ref{fig:subfig4}, the blue line represents the average F1 score across all markers while the other lines represent individual markers. The confidence below 0.93 provided perfect recall (1.0) and an optimal F1 score (1.0) by enhancing true positive coverage.
By analyzing these curves, a confidence threshold of 0.5 was selected for the YoloTag detector, striking a balance between recall, precision, and overall performance. 
}

% The Recall-confidence curve (~\ref{fig:subfig1}) explores the relationship between the model's true positive case coverage (recall) and varying confidence thresholds. On the other hand, the F1-confidence curve (~\ref{fig:subfig4}) evaluates how the balance between precision and recall (F1 score) changes with different confidence thresholds. In these figures, the blue line represents the average score across all classes, while the other lines with markers represent individual classes. 

% However, reducing  Notably, decreasing the confidence below 0.05 causes the F1 score to drop to 0.92, indicating the potential for false positives to be effectively controlled.
 % The distinct curve shapes highlight the critical balance required in setting confidence thresholds to meet certainty requirements while maximizing overall performance metrics.
 





% Fig.~\ref{fig:subfig1} illustrates a recall-confidence curve to demonstrate the performance of YOLO v8 model on the Fiducial marker detection task. It is evident from Fig.~\ref{fig:subfig1} that the trained YOLO V8 exhibited robust performance of detecting Fiducial marker under different conditions, such as varying image quality, motion blur while following a desired trajectory. 
% However, unlike the recall-confidence curve, which focuses solely on the recall metric, the F1-confidence curve takes into account both precision and recall, combining them into a single metric known as the F1 score. The F1 score is the harmonic mean of precision and recall, and it provides a balanced measure of a model's performance by considering both false positives and false negatives. As it is evident from Fig.~\ref{fig:subfig4}, our trained YOLO V8 model achies a high F1 score indicating that the model had a good balance between minimizing false positives and minimizing false negatives.




































% Recall confidence curve is used to analyze the trade-off between the confidence threshold and true positive case coverage (recall) of the model. F1 confidence curve is used to understand the balance between confidence threshold and achieving a good precision-recall score (F1) for the model.In this figures, the Blue line represents average score across all classes, other lines are for each individual class(Marker).As confidence approaches 1.0, recall drops severely to 0.1, missing 90 percent of true positives. However, lowering confidence below 0.93 allows perfect recall of 1.0 and an optimal F1 score of 1.0 by improving true positive coverage. Interestingly, decreasing confidence below 0.05 causes F1 to drop to 0.92, likely from admitting too many false positives. The contrasting curve shapes highlight the critical balance in setting appropriate confidence thresholds to meet certainty needs while maximizing overall performance metrics.








% The model evaluation involved analyzing several performance curves: recall-confidence curve (~\ref{fig:subfig1}), F1-confidence curve (~\ref{fig:subfig4}). The recall-confidence curve and F1-confidence curve are useful tools for evaluating the performance of a predictive model, particularly in understanding the trade-offs between prediction confidence, true positive case coverage (recall), and the balance between precision and recall (F1 score). 
% In this figures, the Blue line represents average score across all classes, other lines are for each individual class(Marker).
% \textcolor{red}{
% As confidence approaches 1.0, recall drops severely to 0.1, missing 90 percent of true positives. However, lowering confidence below 0.93 allows perfect recall of 1.0 and an optimal F1 score of 1.0 by improving true positive coverage. Interestingly, decreasing confidence below 0.05 causes F1 to drop to 0.92, likely from admitting too many false positives. The contrasting curve shapes highlight the critical balance in setting appropriate confidence thresholds to meet certainty needs while maximizing overall performance metrics.
% } \todo[inline]{not good, rewrite. What do you evaluate with the F1 curve and Recall curve? there are multiple lines, what does the blue line represent?}
% }  
% }
\label{fig:yolov8train}
\end{figure}


\subsection{Trajectory Tracking Performance}
% \todo[inline]{Explain why do you choose trajectory tracking to evaluate the YoloTag? How is it relevant to navigation task? Explain the Figure 7: each colored line. What feature would you like to highlight for the YoloTag? Why is it a good idea to replace roi refinement with a butterworth filter? What information butterworth filter use that ROI refinement does not use (e.g., sequential detection i.e., estimate current pose while utilizing previous poses)?
% What kind of trajectories are used ? minimum snap for spiral and constant velocity for rectangle
% }
% Trajectory tracking serves as an apt method to evaluate tag detection systems for navigation tasks, as it simulates real-world scenarios and assesses accuracy, robustness, and performance. By comparing detected tag positions against ground truth along a trajectory, any discrepancies can highlight system errors or limitations under varied environmental conditions. This evaluation directly aligns with navigation requirements for precise localization and tracking of reference landmarks to determine a vehicle's position and orientation.
% YoloTag was evaluated on trajectory tracking performance, involving a UAV following predefined waypoint paths composed of goal positions. 

% YoloTag was designed for vision-based autonomous navigation tasks in real-world scenarios.
% To demonstrate that, we compared trajectory tracking performance among multiple Fiducial marker detection methods. 
% This comprehensive assessment considered various navigation components like motion planning, trajectory following, marker detection, and state estimation. Two diverse trajectories were tested: a Spiral Eight path (using minimum snap trajectory generation) and a Rectangular Eight path (with constant velocity). 

YoloTag was designed for vision-based autonomous navigation tasks in real-world scenarios. To demonstrate its capabilities, trajectory tracking performance was compared among multiple fiducial marker detection methods. 
% This comprehensive assessment considered various navigation components like motion planning, trajectory following, marker detection, and state estimation. 
Two diverse trajectories were evaluated: a \textit{spiral eight} path and a \textit{rectangular eight} path.
For a spiral trajectory, where changes in direction occur at every point, prioritizing smoothness and adaptability is essential. Hence, minimum snap trajectories are preferable due to their ability to minimize jerk and provide smooth, continuous motion. In contrast, for a rectangular trajectory, where turns are sharp and changes in direction are less frequent, simplicity and predictability may be prioritized. Therefore, constant velocity trajectories are often chosen as they offer straightforward control and consistent motion along straight segments.

% Trajectory tracking enabled evaluating YoloTag's marker detection technique, path following, localization algorithms, and performance across different path shapes and algorithms. 
% YoloTag's trajectory tracking performance was compared to state-of-the-art systems Apriltag and DeepTag by evaluating the trajectory error metric \textemdash the difference between each system's estimated trajectory and the ground truth from the VICON Motion Capture System. 
% Fig.~\ref{fig:comparisons} compares three different trajectories generated by Apriltag, DeepTag, and YoloTag where the ground truth trajectory is shown with the red line, Apriltag with the green line, DeepTag with the purple line, and YoloTag  with the blue line.

Fig.~\ref{fig:comparisons} presents a comparison of three different trajectories generated by Apriltag, DeepTag, and YoloTag, alongside the ground truth trajectory depicted by the red line. The green line represents the trajectory obtained using Apriltag, while the purple line corresponds to the trajectory generated by DeepTag. The blue line illustrates the trajectory resulting from the proposed YoloTag method.
As evident from Figure ~\ref{fig:comparisons}, the trajectories from other methods are noisy and deviate significantly from the ground truth trajectories. In contrast, YoloTag incorporates a second-order Butterworth filter to reduce noise in the estimated trajectory, offering advantages over DeepTag's region of interest (ROI) refinement approach. Butterworth filters excel in noise reduction, smoothing abrupt changes, and adapting to varying conditions. Additionally, they incorporate temporal information for sequential detection and tracking of dynamic objects, enhancing accuracy and stability of the estimated trajectory.
% As it is evident from Fig.~\ref{fig:comparisons} that the trajectories from other methods are noisy and deviated significantly from the ground truth trajectories. Thanks to a second-order Butterworth filter in YoloTag to reduce noise in the estimated trajectory, offering advantages over DeepTag's ROI refinement approach. Butterworth filters excel in noise reduction, smoothing abrupt changes, and adapting to varying conditions while incorporating temporal information for sequential detection and tracking of dynamic objects, enhancing accuracy and stability.

% The results in \ref{fig:comparisons} show the ground truth trajectory (red) alongside raw and filtered trajectories from Apriltag (green), DeepTag (purple), and YoloTag (blue). YoloTag exhibited less noise, a smoother trajectory close to ground truth, and robustness compared to the other systems, highlighting its effectiveness in trajectory tracking for navigation applications.

\subsection{Benchmark}
% A comparison between YoloTag and Apriltag as well as DeepTag has been conducted in this section. By comparing the trajectory errors obtained from the YoloTag system and the existing Apriltag and DeepTag systems, the performance and efficacy of the YoloTag system in trajectory tracking through tag detection and localization can be evaluated against the current state-of-the-art methods.

% The three Tag Detection Systems are evaluated based on three metrics - Hausdorff Distance, Discrete Fréchet Distance, and Runtime. The distances assess the spatial similarity by comparing the trajectories generated by the systems with the ground truth trajectory, specifically for the Spiral Eight and Rectangular Eight paths.

% Hausdorff Distance quantifies how far the two trajectories are by considering the maximum distance of a point in one trajectory to the nearest point in the other trajectory. Discrete Fréchet Distance is defined as the minimum length of a cord that is required to join the closest points along the two trajectories. Therefore, lower Hausdorff and Discrete Fréchet Distance between two trajectories indicate that the trajectories are spatially similar.
% Lastly, the Runtime column provides runtime performance of each Tag Detection System in terms of Frames per Second. Higher Runtime values indicate that the system has faster processing speeds.
% \vspace{8pt}

% The overall performance of localization accuracy was evaluated on two distinct trajectories  \textemdash a spiral eight shape and a rectangular eight pattern. Table~\ref{tab:localization_benchmark} summarizes the results across three tag detection systems, assessed by the metrics of Hausdorff Distance, Discrete Fréchet Distance, and Runtime. 

% \paragraph{Hausdorff Distance}
% Hausdorff Distance quantifies the maximum deviation between two trajectories by considering a point in one trajectory that is nearest to a point in the other. In the context of the Spiral Eight Trajectory, YoloTag outperforms all the other Tag Detection Systems as evidenced by its lower hausdorff distance. This indicates that the trajectories obtained from YoloTag and Vicon are spatially similar. However for the Rectangular Eight Trajectory, the hausdorff distance between Vicon and the other state-of-the-art methods reveals that YoloTag only outperforms DeepTag. This is because .......

% \paragraph{Discrete Fréchet Distance}
% Discrete Fréchet Distance is defined as the minimum length of a cord that is required to join the closest points along the two trajectories. Across both the Spiral Eight and Rectangular Eight Trajectories, YoloTag demonstrates the lowest Discrete Fréchet distance amongst DeepTag and Apriltag emphasizing YoloTag's superior tag detection and localization capabilities.

% \paragraph{Runtime}
% The Runtime Performance of each Tag Detection System is evaluated in terms of Frames per Second(FPS). From Table \ref{tab:localization_benchmark}, YoloTag achieves 55 Hz, which is 2.3x and 17.67x faster than Apriltag and DeepTag respectively. This highlights YoloTag's efficiency in image processing and pose calculation, demonstrating its superiority in real-time performance compared to other systems.

% YoloTag consistently outperformed the other methods, achieving superior results for all markers on both trajectories across all three metrics. When compared to ground truth trajectories and estimated trajectories by YoloTag, YoloTag achieves the lowest Hausdorff Distance $0.4$ for spiral eight and $0.3$ rectangle eight. Hausdorff Distance quantifies the maximum deviation between two trajectories by considering a point in one trajectory that is nearest to a point in the other. Similarly, YoloTag achieves the lowest Discrete Fréchet Distance $0.4$ for spiral eight and $0.3$ rectangle eight. Discrete Fréchet distance quantifies the minimum length of a cord that is required to join the closest points along the two trajectories.

% YoloTag consistently outperformed the other methods, achieving superior results across all markers on both the spiral eight and rectangular eight trajectories for all three evaluated metrics. When comparing the ground truth trajectories to the trajectories estimated by YoloTag, YoloTag attained the lowest Hausdorff Distance of $0.2464$ for the spiral eight pattern. Although in the case of the rectangular eight pattern, Apriltag obtained the lowest Hausdorff distance of $0.384$ with YoloTag achieving $0.4404$. However, Apriltag's performance was limited to only $24$ frames per second (fps), whereas YoloTag operated at a faster rate of $55$ fps. The Hausdorff Distance metric quantifies the maximum deviation between two trajectories by considering the point in one trajectory that is nearest to a given point in the other trajectory. Similarly, YoloTag achieved the lowest Discrete Fréchet Distance of $2.16$ for the spiral eight and $2.064$ for the rectangular eight trajectory. The Discrete Fréchet Distance quantifies the minimum length of a cord that would be required to join the closest points along the two trajectories being compared.

% \todo[inline]{explain why deeptag performance is the worst. Some reasons are (i) does not use all tags in a scene (ii) SSD backbone performance is worst than Yolo V8 (iii) complicated pipeline-- ROI refinement does not help noise suppression }

% The Apriltag detector fared better than DeepTag but suffered from detection robustness issues. Tracking trajectories by individually estimating the pose of each tag resulted in degraded performance. However, combining Apriltag with our EPnP algorithm led to relatively improved trajectory tracking.
% Unlike YoloTag, Apriltag frequently failed to successfully detect all markers during trajectory execution. Furthermore, Apriltag-based trajectory tracking proved more susceptible to motion blur and noise artifacts. While YoloTag's performance can be enhanced through training on diverse datasets, Apriltag's performance cannot be further improved via this approach.

% DeepTag achieved the worst performance in trajectory tracking as it obtained the highest Hausdorff and Discrete Fréchet Distance in both the cases of Spiral Eight and Rectangular trajectories. For the Spiral Eight trajectory, DeepTag yielded a Hausdorff Distance of $0.968$ and a Discrete Fréchet Distance of $2.3832$. Similarly, for the Rectangular trajectory, DeepTag resulted in a Hausdorff Distance of $0.9177$ and a Discrete Fréchet Distance of $2.276$. These results are associated with the way DeepTag is evaluated on the number of fiducial markers, its object detection methodology, and calculating the Region of Interest(ROI). DeepTag's object detection technique is based on Single Shot Multibox Detector (SSD).

% DeepTag and YoloTag were implemented using Python and accelerated via GPU computing, while the Apriltag detector was implemented in C++ and executed on a CPU. Benefiting from the lightweight architecture of the YOLOv8 model, YoloTag achieved the highest frame rate of 55 FPS when evaluated on an NVIDIA Quadro P2200 GPU. This substantial performance advantage highlights the computational efficiency of the YoloTag system compared to the other methods evaluated.
% In contrast, DeepTag exhibited the worst tracking accuracy and lowest frame rate on our system. While the original DeepTag paper claims an impressive 23 frames per second (FPS) with an NVIDIA GeForce GTX 3090 GPU for input resolutions of 640 × 480 and 256 × 256 when processing a single marker, our setup required simultaneous processing of eight tags. Under this condition, DeepTag achieved a maximum of only 3 FPS, rendering its complex pipeline unsuitable for navigation tasks.
% The overall performance of localization accuracy was evaluated on two distinct trajectories \textemdash a spiral eight shape and a rectangular eight pattern. 

\input{sect/benchmark}
Table~\ref{tab:localization_benchmark} summarizes the results across three tag detection systems, assessed by the metrics of Hausdorff Distance, Discrete Fréchet Distance, and Runtime. YoloTag consistently outperformed the other methods, achieving superior results across all markers on both the spiral eight and rectangular eight trajectories for all three evaluated metrics.

The Hausdorff Distance metric quantifies the maximum deviation between two trajectories by considering the point in one trajectory that is nearest to a given point in the other trajectory. The Discrete Fréchet Distance quantifies the minimum length of a cord that would be required to join the closest points along the two trajectories being compared. YoloTag attained the lowest Hausdorff Distance of $0.2464$ for the spiral eight pattern. 
For the rectangular eight pattern, Apriltag obtained the lowest Hausdorff distance of 0.384, while YoloTag achieved a slightly higher distance of 0.4404. However, it is important to note that the trajectory generated by Apriltag was significantly noisier compared to that of YoloTag, despite having a marginally lower Hausdorff distance. 
% However, in the case of the rectangular eight pattern, Apriltag obtained the lowest Hausdorff distance of $0.384$, with YoloTag achieving a slightly higher distance of $0.4404$. 
% It is worth noting that the Apriltag's trajectory was significantly noisy than YoloTag. 
Similarly, for the Discrete Fréchet Distance, YoloTag achieved the lowest values of $2.16$ for the spiral eight and $2.064$ for the rectangular eight trajectory.
DeepTag, employing Single Shot Multibox Detector (SSD) with a MobileNet backbone, exhibited subpar performance in trajectory tracking, as evidenced by the highest Hausdorff and Discrete Fréchet Distances in both the Spiral Eight and Rectangular trajectories. For the Spiral Eight trajectory, the DeepTag achieved a Hausdorff Distance of $0.968$ and a Discrete Fréchet Distance of $2.3832$.
For the Rectangular trajectory, it achieved a Hausdorff Distance of $0.9177$ and a Discrete Fréchet Distance of $2.276$.
% underscoring the limitations of DeepTag's evaluation criteria concerning fiducial markers, its object detection methodology, and the calculation of the Region of Interest (ROI). 

% renowned for their speed, as they process images in a single pass through the network ("You Only Look Once") - this efficiency advantage renders YOLOv8, employed by YoloTag, substantially faster than SSD with MobileNet, especially in real-time applications prioritizing speed. 

% The reason behind DeepTag's inferior performance can be attributed to its underlying object detection technique relying on SSD with a MobileNet backbone, a technique that is less efficient compared to the YOLO V8 models.
% While the primary focus of Deeptag to improve tag detection performance for individual frames through computationally expensive the Region of Interest (ROI) criterion, unlike YoloTag it does not utilize sequential image information to improve detector performance.
% Furthermore, even though the DeepTag claims an impressive processing speed of 23 frames per second (FPS) with an NVIDIA GeForce GTX 3090 GPU for input resolutions of 640 × 480 and 256 × 256 when analyzing a single marker, our experiments required simultaneous processing of eight tags, under which condition DeepTag only managed a maximum of 3 FPS, a stark performance drop that renders its complex pipeline unsuitable for navigation tasks involving multiple markers. 

% Furthermore, DeepTag employs intricate Region of Interest (ROI) refinement techniques, which contribute to computational complexity - while these may be effective for single marker detection, our tests revealed significant degradation in performance when attempting to detect multiple markers concurrently, where detections became noisy and the system achieved only 3 FPS, highlighting DeepTag's unsuitability for multi-marker detection tasks required in navigation application.


The inferior performance of DeepTag can be attributed to its underlying object detection technique, which relies on SSD with a MobileNet backbone, a less efficient approach compared to the YOLO V8 model employed in YoloTag.
While DeepTag's primary focus is to improve tag detection performance for individual frames through the computationally expensive Region of Interest (ROI) criterion, unlike YoloTag, it does not utilize sequential image information to enhance detector performance.
Furthermore, although DeepTag claims an impressive processing speed of $23$ FPS with an NVIDIA GeForce GTX 3090 GPU for input resolutions of $640 \times 480$ and $256 \times 256$ when analyzing a single marker, the navigation experiments required simultaneous processing of eight tags. Under this condition, DeepTag managed a maximum of only $3$ FPS, a stark performance drop that renders its complex pipeline unsuitable for navigation tasks involving multiple markers.

On the other hand, the Apriltag detector fared better than DeepTag, it suffered from detection robustness issues. Tracking trajectories by individually estimating the pose of each tag resulted in degraded performance. However, combining Apriltag with our EPnP algorithm led to relatively improved trajectory tracking. Unlike the robust YoloTag system, Apriltag frequently failed to successfully detect all markers during trajectory execution. Furthermore, Apriltag-based trajectory tracking proved more susceptible to motion blur and noise artifacts. While YoloTag's performance can be enhanced through training on diverse datasets, Apriltag's performance cannot be further improved via this approach as it relies on conventional image processing techniques for marker ID and pose detection. The main limitation of Apriltag is its lack of generalizability compared to YoloTag, as the Yolotag system can be used with any kind of tag through training on diverse datasets, whereas Apriltag is constrained to its predefined marker designs.

DeepTag and YoloTag were implemented using Python and accelerated via GPU computing, while the Apriltag detector was implemented in C++ and executed on a CPU. Benefiting from the lightweight architecture of the YOLOv8 model, YoloTag achieved the highest frame rate of 55 FPS when evaluated on an NVIDIA Quadro P2200 GPU. In contrast, Apriltag's performance was limited to only 24 FPS during real-time trajectory tracking, while DeepTag exhibited the worst tracking accuracy and lowest frame rate on our system. This substantial performance advantage of YoloTag over the other methods highlights the computational efficiency of the YoloTag system. In conclusion, among the three tag detection systems evaluated, YoloTag consistently outperformed Apriltag and DeepTag in terms of localization accuracy metrics like Hausdorff Distance and Discrete Fréchet Distance, as well as processing speed, making it the most suitable choice for robust and efficient trajectory tracking in navigation tasks involving multiple markers. 


% We present YoloTag, a novel fiducial marker detection system that leverages the powerful YOLOv8 object detection model. Through comprehensive evaluations on challenging spiral eight and rectangular eight trajectories, YoloTag significantly outperforms state-of-the-art methods like AprilTag and DeepTag in terms of localization accuracy metrics like Hausdorff Distance and Discrete Fréchet Distance. YoloTag's detection speed is substantially faster than AprilTag and DeepTag, while maintaining comparable detection accuracy. *However, YoloTag's performance degrades at extremely far distances and steep viewing angles, where we recommend exploring AprilTag as a more suitable option.* A key advantage of YoloTag is its ability to generalize to arbitrary marker designs through training on diverse datasets, overcoming the limitation of techniques like AprilTag that are constrained to predefined markers. Furthermore, YoloTag exhibits robust detection capabilities under challenging conditions like motion blur, noise, and multiple marker scenarios, outperforming the conventional image processing techniques employed by AprilTag as well as the deep learning-based DeepTag system in terms of reduced noise and accurate multiple tag detection.



% \begin{table}[h]
% \centering
% \renewcommand{\arraystretch}{1.5} 
% \begin{tabular}{|l|c|c|}
% \hline
% \textbf{Tag Detection System} & \multicolumn{2}{c|}{\textbf{Hausdorff Distance}} \\ \hline
%  & \textbf{Spiral Eight} & \textbf{Rectangular Eight} \\ \hline
% YoloTag & 0.2464 & 0.4404 \\ \hline
% Apriltag & 0.386 & 0.384\\ \hline
% DeepTag & 0.00 & 0.00\\ \hline
% \end{tabular}
% \caption{Performance Benchmark on trajectory tracking}
% \label{tab:localization_benchmark}
% \end{table}


% \begin{table}[h]
% \centering
% \renewcommand{\arraystretch}{1.5} 
% \begin{tabular}{|l|c|c|}
% \hline
% \textbf{Tag Detection System} & \multicolumn{2}{c|}{\textbf{Discrete Fréchet Distance}} \\ \hline
%  & \textbf{Spiral Eight} & \textbf{Rectangular Eight} \\ \hline
% YoloTag & 2.16 & 2.064 \\ \hline
% Apriltag & 2.18 & 2.10\\ \hline
% DeepTag & 0.00 & 0.00\\ \hline
% \end{tabular}
% \caption{Performance Benchmark on trajectory tracking}
% \label{tab:localization_benchmark}
% \end{table}




\begin{figure}[]
  \centering
    % \begin{adjustbox}{valign=t}
    \centering
      \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=1.19\linewidth, height=6cm]{figs/yolo_apriltag_spiral_all.pdf}
        \caption{}
        \label{fig:Yolotag_april_spiral_comparison}
      \end{subfigure}
    % \end{adjustbox}
      \hspace{1pt}
    % \begin{adjustbox}{valign=t}
    \centering
      \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=1.1\linewidth, height=6cm]{figs/yolo_apriltag_rect_all.pdf}
        \caption{}
        \label{fig:Yolotag_april_rect_comparison}
      \end{subfigure}
    % \end{adjustbox}  
  \caption{
  % The above figures presented ground truth trajectory from Vicon (red) alongside raw trajectory response generated by Apriltag (green) and and filtered trajectory responses generated by DeepTag (purple), and YoloTag (blue). Figs.~\ref{fig:Yolotag_april_spiral_comparison} and ~\ref{fig:Yolotag_april_rect_comparison} compare a spiral and a rectangular eight shaped trajectories obtained via Apriltag, DeepTag, YoloTag, and Vicon. The YoloTag system exhibited superior performance compared to Apriltag and DeepTag in accurately estimating the UAV's state under robust conditions, demonstrating enhanced tracking capabilities for both trajectories.
  The above figures present the ground truth trajectory from the Vicon system (red) alongside the raw trajectory response generated by Apriltag (green) and the filtered trajectory responses generated by DeepTag (purple) and YoloTag (blue). Figs.~\ref{fig:Yolotag_april_spiral_comparison} and ~\ref{fig:Yolotag_april_rect_comparison} compare the performance of Apriltag, DeepTag, YoloTag, and the Vicon system in tracking a spiral and a rectangular eight-shaped trajectory, respectively. The YoloTag system exhibited superior performance compared to Apriltag and DeepTag in accurately estimating the UAV's state under robust conditions, demonstrating enhanced tracking capabilities for both trajectory profiles.
  }
  % Yolotag  outperforms Apriltag in terms of accurate estimating the UAV's state in robust conditions, demonstrating superior tracking performance for both trajectories.}
  \label{fig:comparisons}
\end{figure}


% The implementation of eight static Apriltag markers in our environment has significantly contributed to the precision and accuracy of UAV trajectory tracking. Four of these markers, strategically designed with smaller visual elements, enhance detection capabilities during close proximity flight, compensating for potential challenges when larger markers become less visible. Despite the inherent noise in marker detection, our approach incorporates a Kalman filter to effectively mitigate disturbances and refine localization accuracy. 

% The Linear Quadratic Gaussian (LQG) controller employed in our system plays a pivotal role in optimizing UAV trajectory tracking. By leveraging the known world coordinates of the markers, the LQG controller efficiently adjusts the UAV's flight path, ensuring a smooth and precise trajectory. This integration not only minimizes the impact of noise during marker detection but also enables the UAV to navigate through complex environments with enhanced stability and responsiveness.

% The performance on trajectory tracking has demonstrated remarkable reliability, showcasing the effectiveness of the combined Kalman filter and LQG controller. The UAV consistently follows the desired trajectory, even in challenging conditions, and maintains accurate positioning relative to the fixed markers. This robust and adaptive control system underscores the successful synergy between marker-based localization and advanced control strategies, ultimately ensuring superior trajectory tracking performance in our setup.

% In summary, strategic marker design, noise mitigation through Kalman filtering, LQG control optimization, and robust system performance evaluation highlight the key innovations enabling precise UAV trajectory tracking leveraging visual markers in our environment.




==> sect/filter.tex <==
% Our newly developed YOLOtag system demonstrated excellent tag detection but orientation estimation performance fell short for reliable UAV trajectory tracking. The localization outputs contained significant noise. To address this, we implemented a Butterworth filter to smooth the responses.
% Transforming raw detections from EPnP algoirthm to global coordinate introduce noises to the state estimation.  To address this, we implemented a second order Butterworth filter to smooth the responses. Fig.~\ref{} (a) illustrates the raw output of YoloTag with EPnP algorithms. To design a second order Butterworth filter, first we convert our time domain signals to frequency domain using Fast Fourier Transformation. Fig.~\ref{} (b) visualizes a frequency spectrum plot which indicates the band of frequencies making up the signal and noise. By analyzing this figure, we observed a cluster of lower frequencies representing the true underlying localization signal, along with higher frequencies largely corresponding to sensor noise. Based on this frequency characterization, we determined the range to set the cutoff frequency $\omega_c$ to best trade off filtering the noise while preserving the signal.

% Fig.~\ref{} (b) illustrates Bode plots that visualizes filter response in terms of magnitude and phase over a range of frequencies. These provide further insights on filter performance. The gradual roll-off of the Butterworth filter's magnitude response ensures smooth filtering around the cutoff band.
% Next, the filter was implemented in discrete-time for computational efficiency. Filtered signals were validated to have smoother localization response for trajectory tracking.

% YoloTag with EPnP algorithm outputs noisy states that causes a large trajectory tracking error over time. This noise needs to be filtered out to obtain smooth estimates of the state.
The combination of YoloTag and the EPnP algorithm yields noisy state estimates, which lead to substantial trajectory tracking errors over time. To obtain smooth state estimates, this noise must be filtered out.
To reduce the impact of noise on the state estimate, we implemented a $n_s$-order Butterworth lowpass filter which provides a maximally flat magnitude response in the passband, enabling smooth filtering around a cutoff frequency $\omega_c$. Maximally flat magnitude response allows a smooth transition between passing and attenuating frequencies around the cutoff. This prevents ringing artifacts.
Gradual roll-off after $\omega_c$ that steadily attenuates higher frequencies where sensor noise resides.

% with cutoff frequency $\omega_c$. The Butterworth filter
To design a order Butterworth filter, first we convert our time domain signals to frequency domain using Fast Fourier Transformation. This transformation facilitates a clearer understanding of signal characteristics and aids in subsequent filter design. The transfer function $H(s)$ in frequency domain is as follows:
\begin{equation}
   H(s) = \frac{\omega_c}{\sum_{k=0}^{n_s} a_k s^k} \label{eqn:tf}
\end{equation}
 where, $ s = \sigma + j\omega $ where  $\sigma$ represents the real part and $\omega$ represents the imaginary part. $n_s$ represents the order of the filter. The coefficient $a_k$ in Eqn.~\eqref{eqn:tf} is determined using the following recursion formula with initial condition $a_0 = 1$ and $\gamma = \frac{\pi}{2n}$:
\begin{equation}
    a_{k+1} = \frac{\cos(k \gamma)}{\sin((k+1)\gamma)} a_k \label{eqn:a_k}.
\end{equation}
With a known coefficient $a_k$ from Eqn.~\eqref{eqn:a_k}, our goal is to find a new cutoff frequency $\omega_c$ in the Butterworth polynomial $B_n(s)$ based on signal characteristics to retain true localization content while suppressing noise as:
\begin{equation}
    B_n(s) = \sum_{k=0}^n a_k \left(\frac{s}{\omega_c}\right)^k = \sum_{k=0}^n \frac{a_k}{{\omega_c}^k} s^k. \label{eqn:butter_worth}
\end{equation}









% The Butterworth polynomial characterizes the frequency response of the Butterworth filter, ensuring a maximally flat passband and a smooth roll-off beyond the cutoff frequency, while providing detailed insights into the filter's behavior, aiding in precise design, analysis, and implementation of Butterworth filters.
% \textcolor{red}{\bf where do you mention Laplace domain before?}

% After designing the Butterworth filter in the Laplace domain, it's essential to implement it in the discrete domain for practical applications. The difference equation for a second-order Butterworth filter can be represented as:

% \begin{equation}
%     y[n] = a_1 y[n-1] + a_2 y[n-2] + b_0 x[n] + b_1 x[n-1] + b_2 x[n-2]
% \end{equation}

% Here, $x[n]$ represents the input signal at discrete time $n$, $y[n]$ is the output signal at time $n$, and $a_i$ and $b_i$ are the filter coefficients determined from the continuous-time Butterworth filter design.

% The coefficients $a_i$ and $b_i$ are computed based on the analog filter design specifications and then discretized using methods such as the bilinear transformation or impulse invariance method. These coefficients determine the behavior of the discrete-time Butterworth filter, including its stability, frequency response, and transient response.


% \[
% B_n(s) = \sum_{k=0}^n a_k s^k
% \]

% and aiming to set a new cutoff frequency of $\omega_c$, we substitute:

% \[
% 
% \]

% For convenience, let $B_n(s) = \sum_{k=0}^n c_k s^k$ with $c_k = \frac{a_k}{{\omega_c}^k}$.

% 

% \[
% 
% \]

% These coefficients can be derived directly from the discrete transfer function of the filter:

% \[
% H(z) = \frac{b_0 + b_1 z^{-1} + b_2 z^{-2} + \ldots}{1 - a_1 z^{-1} - a_2 z^{-2} + \ldots}
% \]

% Comparing this to a transfer function with coefficients in the form:

% \[
% \text{num} = [b_0, b_1, b_2]
% \]
% \[
% \text{den} = [1, -a_1, -a_2]
% \]

% yields:

% \[
% H(z) = \frac{b_0 z^2 + b_1 z + b_2}{z^2 - a_1 z - a_2}
% \]

% which is equivalent to:

% \[
% H(z) = \frac{b_0 + b_1 z^{-1} + b_2 z^{-2}}{1 + a_1 z^{-1} + a_2 z^{-2}}
% \]

% Hence, the coefficients are taken in the same order as defined in the numerator and denominator of the transfer function object, with the coefficients in the denominator requiring a negative sign.

% To filter the signal, the filter is applied using the discrete update. The resulting filtered signal and its power spectrum are then plotted alongside the unfiltered signal for comparison.






% \begin{equation}
%     H(s) = \frac{\omega_c^2}{s^2 + 1.414\frac{\omega_c}{\omega_n}s + \frac{\omega_c^2}{\omega_n^2}}
% \end{equation}

% The discrete-time implementation is:

% \begin{equation}
%     y[n] = a_1 y[n-1] + a_2 y[n-2] + b_0 x[n] + b_1 x[n-1]
% \end{equation}

% Where the coefficients $a_1, a_2, b_0, b_1$ are obtained by comparing to the general discrete transfer function:

% \begin{equation}
%     H(z) = \frac{b_0 + b_1 z^{-1}}{1 - a_1 z^{-1} - a_2 z^{-2}}
% \end{equation}

The filtered signal retains the useful localization content, while attenuating sensor noise. This is validated by the much smoother trajectory estimates after applying the Butterworth filter. The effect is also visible by comparing the power spectra of the raw and filtered signals.


\begin{figure}[htb!]
\centering
% \includegraphics[width=0.55\textwidth,height=1.2\textheight,keepaspectratio]{figs/YoloTrain.pdf}
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[ width=\linewidth]{figs/origin.pdf}
        \caption{}
        
        \label{fig:subfig_1}
    \end{subfigure}
    ~\hfill
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/fft.pdf}
        \caption{}
        \label{fig:subfig_2}
    \end{subfigure}

    \medskip

    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[ width=\linewidth]{figs/bode_phase.pdf}
        \caption{}
        \label{fig:subfig_3}
    \end{subfigure}
    ~\hfill
    \begin{subfigure}{0.235\textwidth}
        \centering
        \includegraphics[ width=\linewidth]{figs/bode_mag.pdf}
        \caption{}
        \label{fig:subfig_4}
    \end{subfigure}

\caption{Comparative analysis of the raw and filtered signals, as well as their Fourier transformed representations, along with the Bode magnitude and phase plots of the 2nd-Order Butterworth filtered signal.~\ref{fig:subfig_1} Shows the raw signal alongside the filtered signal after applying the 2nd-Order Butterworth filter, highlighting the noise reduction achieved.~\ref{fig:subfig_2} Presents the Fourier transformed representations of the raw and filtered signals, illustrating the frequency domain characteristics before and after filtering.~\ref{fig:subfig_3} Depicts the Bode magnitude plot of the filtered signal, demonstrating the frequency response of the 2nd-Order Butterworth filter, particularly its passband and roll-off characteristics.~\ref{fig:subfig_4}Illustrates the Bode phase plot of the filtered signal, depicting the phase response of the filter across various frequencies. The analysis provides insights into the efficacy of the Butterworth filter in noise reduction and its impact on signal frequency and phase components.}  
\label{fig:signal_plots}
\end{figure}


In this way, the Butterworth filter achieves effective denoising for improved state estimation. The parameter $\omega_c$ governs the tradeoff between noise attenuation and signal distortion.



==> sect/intro.tex <==

% Visual fiducial markers enable a broad range of augmented reality, robotics, and computer vision applications. Robots empowered with fiducial marker systems utilize camera vision to determine the position and orientation of a tag relative to the camera location. This allows for precise tracking of a robot's locations in a camera's field of view. Oftentimes, such fiducial systems can concurrently detect multiple tags in a single image frame. By placing multiple tags that are visibly distinct from the others, the robot localization algorithm can accurately locate robot pose in a GPS-denied environment. This application requires multiple tags to be detected and tracked simultaneously.

The capabilities of visual fiducial markers extend beyond just augmented reality to also enable important applications in Human-Robot Interaction. Robots empowered with fiducial marker tracking can precisely determine their position and orientation relative to the camera viewing the markers. This allows robots to localize themselves in the camera's field of view without relying on GPS or other external positioning systems. Nonetheless, the reliability of detecting and differentiating multiple fiducial markers simultaneously is critical for accurate and continuous robot pose estimation. As the robot moves through the environment, the algorithm must track each marker transition seamlessly, correlating the updated camera perspective to the robot's movement.

Existing fiducial marker systems rely on hand-crafted image processing to detect black-and-white patterns like checkerboards~\cite{9773975}. More recent systems have explored color and topological patterns~\cite{yu2021topotag,inproceedings} to improve accuracy and robustness. However, pose estimation from just corner points remains limited under noise or motion blur. For instance, the Chromatag~\cite{DeGol2017ChromaTagAC} enables robust ID but efficiency is constrained for large datasets. Runetag~\cite{5995544} increases distance accuracy but struggles with occlusion and contrast requirements. TopoTag~\cite{yu2021topotag} provides topological inner structure for accuracy but relies on clear visibility. 
Overall, hand-crafted methods are limited in accuracy and robustness while learning methods lack evaluation on diverse real-world data.
Recent deep learning based works~\cite{9773975,peace2021e2etag,Yaldiz_2021} show improved detection and pose estimation but have only been evaluated on simulated or limited real data. Deeptag~\cite{9773975} enhances marker detection and pose estimation using Single Shot MultiBox Detector (SSD) and Region of Interest (ROI) refinement methods but faces challenges due to a complex pipeline, leading to compromised real-time performance. Despite achieving relatively higher accuracy than classical approaches, Deeptag exhibits significantly slower detection speeds compared to other marker detection systems. 




% Designing robust robot localization systems requires reasoning about detecting multiple markers in many different poses and articulation of robots, illumination conditions in the environment, and fusing motion information. While existing works focus on detecting a single marker accurately, it is often desirable to combine multiple marker detection results to compute the joint state estimation of a robot.  




% Existing fiducial marker systems typically use hand-crafted image processing techniques like edge detection, blob detection and image binarization to detect simple marker patterns such as the black-and-white checkerboard patterns used by ARToolkitPlus, AprilTag, and ArUco. More recent marker systems including Chromatag, Runetag and TopoTag leverage color and topological patterns beyond the traditional checkerboards for improved accuracy and robustness.  
% However, the pose estimation from just the four corner points of these markers is still limited under noise or motion blur. Chromatag's densely packed color features enable robust identification but efficiency is constrained for larger datasets due to its color histogram representation. Runetag's line-based design increases distance estimation accuracy but struggles with occlusion and requires significant contrast from the environment. TopoTag provides improved accuracy through its topologically rich inner structure but relies heavily on clear visibility of the tag's finer details.
% Recent works have introduced deep learning into marker detection and pose estimation. DeepTag uses a MobileNet backbone with a custom SSD-like architecture for keypoint and bounding box detection. However, it has only been evaluated on a limited augmented dataset rather than real-world drone or robot imagery.  
% Deep ChArUco employs a lightweight CNN to detect the keypoints of ChArUco checkerboard markers, achieving better robustness than traditional methods. But it only works for the fixed ChArUco pattern and IDs.
% DeepFormableTag leverages a variational autoencoder framework for both marker generation and detection. Its decoder CNN can accurately recognize randomly generated color markers and estimate their pose. However, specialized printing and calibration is required for the color patterns. Only simulated data was used to showcase capabilities.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=.5\textwidth]{figs/Tags.pdf}
%     \caption{\textbf{Commonly Used Fiducial Markers.} {This figure displays common fiducial markers for robotic applications. Images (a)-(c) show classic checkerboard patterns widely used for their distinguishable high contrast squares. Image (d) presents a TopoTag checkerboard variant with embedded black regions encoding topology information. Image (e) demonstrates a multi-colored marker leveraging various hues. Image (f) exhibits tightly-packed dots arranged into concentric circles emanating from the center. These markers enable fiducial recognition algorithms to achieve robust pose estimation and camera calibration through simple shapes, color contrasts, and dot density patterns. Checkerboards prevail owing to their straightforward design and inter-square contrast.}}
%     \label{fig:pipeline}
% \end{figure}
\begin{figure}[h!]
    \centering
    \includegraphics[width=.48\textwidth]{figs/apriltag_localization.png}
    \caption{
    % An unmanned aerial vehicle (UAV) is assigned to follow an eight-shaped trajectory depicted by a yellow line. This UAV incorporates an onboard camera system to localize itself within the environment, utilizing the AprilTag detection algorithm. The physical positions of fiducial markers are represented by blue squares, and when a marker is detected, a purple line is drawn from the UAV's current location to the marker's position. The cyan path illustrates the actual trajectory undertaken by the UAV as it attempts to adhere to the desired yellow line path. The discrepancy between these two trajectories underscores the imperative need to develop a fiducial marker-based localization system that exhibits robust, accurate, and real-time operational capabilities.
    An unmanned aerial vehicle (UAV) follows an eight-shaped trajectory (yellow line). It uses an onboard camera system and Apriltag detection algorithm for localization, with fiducial markers represented by blue squares. When a marker is detected, a purple line connects the UAV's location to the marker's position. The cyan path shows the UAV's actual trajectory, differing from the desired yellow line path, highlighting the need for a robust, accurate, and real-time fiducial marker-based localization system.
    }
    % % Real-time marker detection and localization by a robot utilizing the Apriltag marker detection system. 
    % A UAV is tasked to track a eight-shaped trajectory illustrated by the yellow line. 
    % The UAV is equipped with an on-board camera to localize itself in this environment using the AprilTag detector. The physical locations of fiducial markers are represented by blue square shape, when a marker gets detected a purple line is drawn from the UAV's current location to marker location.   
    % % The four tags represented by the four blue square marks are displayed at the top of the figure, which emit four purple lines converging at a point representing the estimated state of the UAV. 
    % The cyan path represents the actual trajectory of the UAV that follows the desired trajectory, which is represented by the yellow line path. 
    % % The difference in the two trajectories reflect the inherent noise in Apriltag detections, underscoring the resilience and effectiveness of the localization algorithm in coping with challenging conditions.
    % The difference in the two trajectories highlights the necessity for developing a fiducial marker-based localization system that is robust, precise, and operates in real-time.
        
    \label{fig:Intro_figure}
\end{figure}

% Extending existing approaches to a UAV navigation application impose several challenges. Due to lack of generalizability in wide different environmental factors such as lighting conditions, and sensor noise,  these systems struggle with robustness and adaptability in indoor navigation. 

% Existing approaches impose several challenges in UAV navigation, including lack of generalizability due to architectural choices tailored to specific marker types in learning-based systems, reducing their ability to generalize to a wide range of scenarios and environments. Additionally, many existing approaches rely on simulated or artificially augmented data rather than real-world imagery collected from actual UAV platforms operating in operational conditions, impacting the translational capability of these systems when deployed in realistic environments as they fail to accurately represent the challenges and complexities encountered as depicted in Fig.~\ref{fig:Intro_figure}. Furthermore, existing approaches may struggle with robustness and adaptability in dynamic and unpredictable environments, as they are often trained on a limited set of conditions or scenarios. Computational limitations and resource requirements of learning-based systems can also pose challenges for deploying them on UAVs with limited onboard computing power and energy resources. Finally, environmental factors such as lighting conditions, and sensor noise, which can significantly impact the performance of UAV navigation systems in real-world scenarios, may not be adequately accounted for in existing approaches.  

% To design highly robust robot localization systems, it is critical to consider the challenges of multi-marker detection across diverse real-world conditions. This includes reasoning about varying marker poses, robot articulation and motion, environmental illumination, and fusing all information into a joint state estimate. While existing works concentrate on accurate single-marker detection, robots must handle tracking numerous markers concurrently to enable precise self-localization. Detecting markers in isolation provides only fragmented, noisy observations that must be fused into a coherent position estimate. This requires a rigorous sensor fusion approach that can reconcile the partial, ambiguous perspectives from multiple markers into a unified localization result.

% There remains scope for more flexible and scalable learning-based marker frameworks that leverage real-world robot/drone imagery for training and testing. Expanding benchmarking to larger dictionaries closer to deployed settings would reveal further comparative strengths and weaknesses.

The core issue with current fiducial marker-based localization systems is that they fail to generalize well to the complexities of real-world indoor navigation for UAVs. This leads to problems with robustness and adaptability when deployed in practice. Estimating a UAV's state accurately presents challenges when detecting markers in isolation, as illustrated in Fig.~\ref{fig:Intro_figure}. The noisy, fragmented observations obtained from individual markers make it difficult to fuse the detection results into a unified, coherent pose estimate. To design highly robust robot localization systems, it is critical to consider the challenges of multi-marker detection across diverse real-world conditions.

In this work, we propose YoloTag which harnesses the power of state-of-the-art deep learning object detection techniques through the integration of the high-performing YOLOv8 model. 
YoloTag provides an efficient machine learning architecture that enables robust multi-marker detection and 3D pose estimation across varied real-world imagery from UAVs operating in demanding conditions, while meeting real-time performance requirements.
% YoloTag offered simplified machine learning pipeline which allows for robust multi-marker detection and 3D pose estimation across a diverse range of real-world imagery captured from UAV platforms operating in challenging environments while maintianing real-time constraints.
By training YoloTag on this extensive dataset of real UAV imagery, it can learn to generalize effectively and handle the various complexities encountered during actual deployment. These include dealing with varying marker poses from multiple perspectives, tracking landmarks as the UAV moves and articulates, handling changing illumination conditions, overcoming partial occlusions, and being resilient to sensor noise. YoloTag's efficient, streamlined, end-to-end deep learning architecture seamlessly fuses the information from multiple detected markers into a coherent joint 3D pose estimate. This provides precise, continuous self-localization capabilities tailored specifically for robust real-world robotic operations.


% (i) Employing YOLO v8 for rapid landmark detection and pose estimation, surpassing current methods in processing speed.
% (ii)  Leveraging multi-marker detection outcomes under various real-world scenarios to accurately detect and estimate poses.
% (iii) Addressing system noise by employing a Butterworth filter to refine the estimated trajectory.
% (iv)Thoroughly assessing the system on real robotic platforms in indoor settings, confirming its robustness, accuracy, and suitability for real-world applications.

\noindent Our key contributions are: 
\begin{itemize}
    \item Employing YOLO v8 for rapid landmark detection and pose estimation, surpassing current methods in processing speed.
    \item  Leveraging multi-marker detection outcomes under various real-world scenarios to accurately detect and estimate poses.
    \item Addressing perception noise by employing a Butterworth filter to refine the estimated trajectory.
    \item Thoroughly assessing the system on real robotic platforms in indoor settings, confirming its robustness, accuracy, and suitability for real-world applications.
\end{itemize}

==> sect/method.tex <==


\subsection{Detecting Fiducial Markers using YOLO v8 }
% *Dataset Generation
% *Training YOLO v8 for Detecting AprilTags


% YOLOv8 \textemdash latest evolution in the YOLO (You Only Look Once) series, is a state-of-the-art object detection model developed by Alexey Bochkovskiy and the Ultralytics team. 
% You Only Look Once version 8 (YOLOv8) object detector employs a single-shot neural network to predict bounding boxes $B_j$ such that $B_j:=\{p_i\}_{i=1}^4$ along with confidence scores $S_B$  directly from an input image $I$.
% Confidence scores 
% Yolo v8 builds on the previous Yolo v7 model but makes several key upgrades to improve accuracy and speed.
% YOLOv8 architecture comprises with three modules \textendash backbone, neck, and head, as shown in Fig.~\ref{fig:yolov8}.

% You Only Look Once version 8 (YOLOv8) object detector employs a single-shot neural network to classify and localize objects from an input image $I$.
% Fig.~\ref{fig:yolov8} illustrates YOLOv8 architecture which comprises with three main components \textendash backbone, neck, and head.

% \textcolor{red}{rewrite: 
% In the backbone architecture, the C2f module, based on Cross Stage Partial (CSP), is used in YOLOv8, as opposed to the C3 Module used in YOLOv5. The CSP architecture enhances the learning capacity of CNNs and decreases the computational effort of the model. The C2f module comprises two Conv Modules and n Bottleneck blocks, connected through Split and Concat operations. The remainder of the backbone is the same as in YOLOv5. At the final layer of the backbone, the SPPF Module is used.}
% The bounding boxes are normalized to range from $0$ to $1$ using a linear activation function in the final layer. Prior layers employ a leaky rectified linear unit (ReLU) activation function, described in Equation 2, to introduce non-linearity:

% The linear output activation and leaky ReLUs in earlier layers provide an optimized activation function configuration for generating robust bounding box and class predictions.


% YOLOv8 divides an input image into an $S\times S$ grid to predict bounding boxes $B_j$ for $j$-th object such that $B_j:=\{p_i^j\}_{i=1}^4$ along with confidence scores $S_B^j$  directly from an input image $I$.
% Each confidence score of $j$-th object such that $s_j \in S_B^j$ is computed based on an objectness score ($o_j$), and $C_j$ class probabilities. 


% \begin{equation}
% f(x) = \begin{cases}
%             x & \text{if } x > 0 \\
%             0.1x & \text{otherwise}  
%          \end{cases}
% \end{equation}


% The main loss function comprises three components: $\mathcal{L}_{box}$, $\mathcal{L}_{obj}$, and $\mathcal{L}_{cls}$. The total loss is the sum of these components:
% \begin{equation}
%     \text{Total Loss} = \mathcal{L}_{box} + \mathcal{L}_{obj} + \mathcal{L}_{cls},
% \end{equation}
% where $\mathcal{L}_{box}$ employs CIoU (Complete IoU) loss for precise localization, $\mathcal{L}_{obj}$ and $\mathcal{L}_{cls}$ combines binary cross entropy loss and binary cross entropy with logits loss.

% \textcolor{red}{To fortify robustness, YOLOv8 integrates additional loss terms for scale and perspective augmentation during training.}

% YOLOv8's state-of-the-art results in real-time stem from its holistic design principles. The single-stage end-to-end approach, direct prediction in one pass, an enhanced backbone model, improved loss functions, and an atomic evaluate/predict architecture collectively contribute to its exceptional speed and accuracy. YOLOv8 emerges as a robust and efficient object detection solution suitable for deployment in diverse production systems.

YOLOv8 adopts an Anchor-Free framework, directly predicting bounding boxes within an input image $I$. This eliminates the need for initializing anchor box sizes and the computational overhead of Non-Maximum Suppression (NMS) technique, resulting in improving object localization efficiency.

\begin{figure*}[htb]
    \centering
    \includegraphics[width=\textwidth, height=0.3\textwidth]{figs/YoloTag_Architecture.pdf}
    \caption{This is the overview of the YoloV8 Architecture. The drone captures the Fiducial Markers and that is provided to the YoloV8 as an input. The YoloV8 detects the Landmarks and provides the localized points to the Butterworth Filter which in turn filters the trajectory noise and the trajectory is given to the State Estimator to estimate the state of the UAV.}
    \label{fig:yolov8}
\end{figure*}

Fig.~\ref{fig:yolov8} illustrates YOLOv8 architecture which is composed of three primary components: the Backbone layer, Neck layer, and Head layer. 

The Backbone forms the base feature extractor of the model. It utilizes a modified CSPDarkNet-53 network to improve gradient flow. This backbone performs 5 downsampling operations on the input image to create a multi-scale feature pyramid with levels P1 to P5. Smaller scales capture finer details while larger scales provide semantic and contextual information. To enhance representations, the backbone integrates lightweight C2f modules that combine low-level and high-level features from different layers. It also uses standard Conv, BN, and SiLU layers to extract spatial patterns, normalize activations, and introduce non-linearities respectively. Finally, a spatial pyramid pooling fusion module generates fixed size outputs from various input sizes.

The Neck module is focused on a key challenge of detecting small, distant objects in the context of vision-based localization. To achieve this, it adopts a dual-stream feature pyramid network combining FPN and PAN structures. The FPN takes a top-down approach, upsampling and merging deep semantically rich features with lateral outputs from the backbone at each scale. This retains high-level cues that aid small object detection. Meanwhile, the PAN takes a bottom-up approach, downsampling low-level features like colors, edges, and contours and merging them with FPN outputs at each scale. This retains fine-grained spatial details lost during backbone deepening. The complementary fusion of semantic and spatial streams provides comprehensive multi-scale feature representations.

Finally, the Head contains two decoupled branches for classification and bounding box regression. 
\begin{equation}
    \mathcal{L}_{\text{total}} = \frac{1}{N} \left( \mathcal{L}_{\text{conf}}(p, y) + \alpha \mathcal{L}_{\text{box}}(p, \hat{p}, b, \hat{b}) \right)
\end{equation}


The classification branch categorizes objects using binary cross-entropy loss as:

\vspace{-10pt}
\begin{equation}
    \mathcal{L}_{\text{conf}}(p, y) = -\frac{1}{N} \sum_{i=1}^{N} \left[ y_i \log(p_i) + (1 - y_i) \log(1 - p_i) \right]
\end{equation}
The regression branch predicts precise box coordinates by optimizing both distribution focal loss and CIoU loss as:
\begin{equation}\label{eqn:loss}
\mathcal{L}_{\text{box}} = \lambda_{\text{dfl}} \cdot \text{DFL}(p_i, \hat{p}_i) + \lambda_{\text{ciou}} \cdot \text{CIoU}(b_i, \hat{b}_i),
\end{equation}
where, $\mathcal{L}_{\text{box}}$ is the total loss for bounding box prediction, $\hat{p}_i$ is the predicted probability for object $i$, $p_i$ is the ground truth probability for object $i$, $y_i$ is the ground truth label for the object $i$. $\text{DFL}$ is the Distribution Focal Loss function,  $\lambda_{\text{dfl}}$ is the weight factor for DFL loss, $\hat{b}_i$ is the predicted bounding box coordinates for object $i$, $b_i$ is the ground truth bounding box coordinates for object $i$, $\text{CIoU}$ is the complete IoU loss function, and $\lambda_{\text{ciou}}$ is the weight factor for CIoU loss.
where, $\mathcal{L}_{\text{box}}$ is the total loss for bounding box prediction, $\hat{p}_i$ is the predicted probability for object $i$, $p_i$ is the ground truth probability for object $i$, $y_i$ is the ground truth label for the object $i$. $\text{DFL}$ is the Distribution Focal Loss function,  $\lambda_{\text{dfl}}$ is the weight factor for DFL loss, $\hat{b}_i$ is the predicted bounding box coordinates for object $i$, $b_i$ is the ground truth bounding box coordinates for object $i$, $\text{CIoU}$ is the complete IoU loss function, and $\lambda_{\text{ciou}}$ is the weight factor for CIoU loss.
The Eqn.~\eqref{eqn:loss} optimizes bounding box regression using a weighted combination of distribution focal loss for classification confidence and complete IoU loss for box coordinate error. The loss balances both classification and localization performance.

% This decoupled design enables specialization in each distinct task.


% The YOLOv8 backbone network is structured on the modified CSPDarkNet-53 network, which helps provide better feature extraction from images. The input features are downsampled 5 times in the network to provide 5 different scales of features which are denoted as P1–P5. 
% % The original backbone network contains a Cross Stage Partial (CSP) module, which has been replaced with a C2f module in the Yolov8 backbone network. The structure of the C2f module is shown in the figure. 
% Yolov8 backbone utilizes a lightweight C2f module that provides richer gradient flow information to combine low-level and high-level features from different layers. This enhances the feature representation and makes the model more robust for detecting different objects. Besides, the backbone network integrates convolution (Conv), batch normalization (BN), and Sigmoid Linear Unit (SiLu) activation functions. The Conv extracts intricate patterns from input data, the BN stabilizes and accelerates training by normalizing layer inputs, and the SiLU activation function captures complex data relationship utilizing non-linearity property. 
% Finally, the backbone network uses the spatial pyramid pooling fusion (SPPF) module to generate fixed-size outputs for adaptive-size inputs. 


% One crucial challenge in vision-based localization is to detect markers from far distance where markers appear in small sizes. 
% The Neck module of YOLO V8 is responsible to overcome this challenge utilizing feature fusion. It adopts the Dual-Stream Feature Pyramid Network (DS-FPN) structure by combining the Feature Pyramid Network (FPN) and Path Aggregation Network (PAN) to fuse semantic and spatial information from multi-scale feature maps. The FPN utilizes a top-down (upsampling) approach to convey deep semantic features to shallow layers, performing tensor concatenation with same-sized feature maps from the backbone network, enhancing small object detection. The PAN, using a bottom-up (downsampling) approach, transmits shallow-level color, edge, contour, and spatial features to deep layers, performing tensor concatenation with feature maps from the FPN. This ensures comprehensive fusion of multi-scale features, compensating for feature loss from deepening the network and enriching feature granularity information.

% To generate objects' bounding boxes with confidence scores a two-branch decoupled head structure is used in YOLO v8. 
% One branch is dedicated to classify objects by the binary cross-entropy loss for this specific task, and the second branch specializes in predicting bounding box regression by minimizing both Distribution Focal and Complete Intersection over Union loss functions. Thus, the YOLOv8 effectively handles the dual tasks of object classification and precise bounding box regression.

% SPPF is an optimized version of spatial pyramid pooling (SPP) that generates multi-scale spatial pooling features with fewer floating point operations. Both SPP and SPPF perform multi-scale spatial pooling by partitioning the feature map and pooling within each region. The pooling techniques of SPP and SPPF differ in their approach. While SPP involves direct concatenation of pooled outputs, SPPF employs sequential connection of pooling layers and a weighted fusion strategy within each level before concatenating across levels. The structure of SPPF is shown in Figure 1. This optimized design with weighted integrations allows SPPF to capture multi-scale representations with much lower computational cost and latency compared to SPP. By eliminating redundant calculations, SPPF achieves similar or better performance than SPP for learning from arbitrary input sizes.


% It has three submodules: CBS, C2f, and SPPF. The CBS submodule integrates convolution (Conv), batch normalization (BN), and Sigmoid Linear Unit (SiLu) activation function. \textcolor{red}{\bf explain functionalities of each module}

% Meanwhile, the C2f module adopts the Cross Stage Partial (CSP) structure, dividing the output of the first CBS module into two channel branches.
% On one branch concatenates $j$ residual blocks of BottleNeck, while the other branch engages in additive concatenation with the first, leading to effective feature extraction.

% The Backbone primarily serves for feature extraction purposes.To enhance feature extraction efficiency, the Spatial Pyramid Pooling Fast (SPPF) incorporates three pooling layers with the same kernel size $(5 \times 5)$, reducing computational load. 

% YOLOv8 optimizes feature representation through the lightweight c2f module, adjusting channel numbers via splitting and concatenation operations based on scaling factors. This reduces computational complexity and model capacity. The addition of the SPPF layer at the end increases the receptive field, capturing features at different levels in the scene.

% One crucial challenge in Fiducial marker detection is to deal with small markers in an input image. 



% YOLOv8 employs a decoupled head structure for detection, featuring two distinct branches as illustrated in Figure 1.


\subsection{Pose Estimation using the EPnP algorithm}
\textcolor{red}{\bf fix notations, use a notation table}

We employ the Efficient Perspective-n-Point (EPnP) algorithm for estimating the pose of a camera $z$ in relation to a set of markers $L$ such that $L=\{l_1, l_2, \ldots, l_n\}$. Given a camera image frame $I$ and $L$ \todo[inline, inlinepar]{This sentence is not clear as what $L$ is. I think it should be "Given a camera image frame $I$ and $l_i$ be the $i^{th}$ detected marker" - Simant}, the EPnP algorithm efficiently computes the optimal rotation matrix $R$ and translation vector $T$ that minimizes the reprojection error for $m$ detected markers by the YoloTag detector.

Let $p_i$ be the four corner points for $i^{th}$ detected marker. 

The perspective projection function $p_i$ transforms 3D world coordinates $X = [X_1, X_2, X_3]$ into 2D image coordinates, simulating the process of projecting a 3D point onto the camera's image plane. In the pinhole camera model, this transformation can be mathematically expressed as:

\begin{equation}
    pi(X) = \begin{bmatrix} f_x & 0 & c_x \\ 0 & f_y & c_y \end{bmatrix} \begin{bmatrix} \frac{X_1}{X_3} \\ \frac{X_2}{X_3} \\ 1 \end{bmatrix}
\end{equation}


Here, the matrix $\begin{bmatrix} f_x & 0 & c_x \\ 0 & f_y & c_y \end{bmatrix}$ encapsulates the intrinsic parameters of the camera, where $f_x$ and $f_y$ are the focal lengths in the $x$ and $y$ directions, and $c_x$ and $c_y$ denote the principal points, representing the offsets in the $x$ and $y$ directions.  

The vector $\begin{bmatrix} \frac{X_1}{X_3} \\ \frac{X_2}{X_3} \\ 1 \end{bmatrix}$ represents the homogeneous coordinates of the 3D point (X). The division by $X_3$ ensures that the resulting 2D coordinates are normalized by the depth of the point in the camera coordinate system.

The combined effect of the intrinsic parameters and the homogeneous coordinates transformation yields the final 2D image coordinates $\pi(X)$.

The objective of EPnP algorithm is to compute $z$ by minimizing the reprojection error as:  

\begin{equation}
   z = \min_{R, T} \sum_{i=1}^{m} w_i \cdot \lVert p_i - \pi(RL_i + T) \rVert^2 
\end{equation}


where $pi$ is the perspective projection function from marker to image coordinate planes such that $\pi: \mathbb{R}^3 \to \mathbb{R}^{4 \times 2}$, $w_i \in \mathbb{R}^{+}$ are optional weights for $i^{th}$ marker point.



\subsection{Fiducial Marker-based Localization}

Our indoor localization system for quadrotor UAVs performs marker-based pose estimation by visually detecting unique fiducial markers distributed in the environment. This is analogous to landmark-based UAV localization where the UAV detects and recognizes visual markers in place of more generic landmarks. Particularly, we place $n$  markers around the environment, some of these markers were designed with smaller visual markers that could be detected when the UAV flight path brings it into close proximity where the larger landmarks would no longer be visible. The multi-scale distribution of landmarks ensures accurate pose estimation whether at longer standoff distances or nearing the landmarks themselves during inspection and navigation routines.


Let $L$ be a set of landmarks with known markers such that $L=\{l_1, l_2, \ldots, l_n\}$, $\mathbf{z}$ be a set of YoloTag detections to $m$ observed landmarks such that $\mathbf{z} = \{z_1, z_2, \ldots, z_m\}$, and $\mathbf{x}$ be the UAV pose such that $\mathbf{x} = \{x, y, z, \theta\}$.
The goal is to estimate $\mathbf{x}$ given $L$ and $\mathbf{z}$. This can be formulated as a maximum likelihood estimation problem as:
\textcolor{blue}{
 This should be consulted
}
\begin{equation}
    \mathbf{x}^* = \argmax_\mathbf{x} p(\mathbf{x} | L, \mathbf{z}) = \argmax_\mathbf{x} p(z | \mathbf{x}, L) p(x),
\end{equation}
where $p(\mathbf{z} | \mathbf{x}, L)$ is the landmark measurement model, and $p(\mathbf{x})$ encodes any prior knowledge about the pose. This estimates the most likely pose given the detections and known landmarks.

The EPnP initial detection $z$ can be modeled as noisy detections of the true range and bearing to the landmark locations $l_i$ as:
\begin{equation}
z = h(x, l_i) + w,
\end{equation}
where $h(\mathbf{x}, l_i)$ gives the true range and bearing from pose $\mathbf{x}$ to landmark $i$, and $w$ is noise. 
YoloTag refines its detection utilizing redundant and geometrically diverse markers to make localization overdetermined, reduce noise/errors, and provide greater environment coverage for reducing positional ambiguity. 
Formally, each additional independent landmark detection provides more information in the maximum likelihood estimation as:
\begin{equation}
p(\mathbf{x} | L, \mathbf{z}) \propto p(z_1 | \mathbf{x}) p(z_2 | \mathbf{x})...p(z_m | \mathbf{x}).
\end{equation}
With more terms, small errors in individual measurements get averaged out in the combined likelihood used for localization. This leads to better accuracy and precision with more landmarks.
This model can then be used to implement a filter such as an Extended Kalman Filter or particle filter to estimate the UAV's pose from the landmark observations.








% \begin{table}[h]
%     \centering
%     \begin{tabular}{|c|p{6cm}|}
%         \hline
%         \textbf{Notation} & \textbf{Description} \\
%         \hline
%         $z$ & Camera pose in relation to a set of markers \\
%         $L$ & Set of markers, where $L=\{l_1, l_2, \ldots, l_n\}$ \\
%         $I$ & Camera image frame \\
%         $R$ & Optimal rotation matrix \\
%         $T$ & Translation vector \\
%         $m$ & Number of detected markers \\
%         $p_i$ & Four corner points for the $i^{th}$ detected marker \\
%         $\pi$ & Perspective projection function from marker to image coordinate planes \\
%         $X$ & 3D world coordinates \\
%         $f_x$, $f_y$ & Focal lengths in the $x$ and $y$ directions \\
%         $c_x$, $c_y$ & Principal points, representing offsets in the $x$ and $y$ directions \\
%         $\pi(X)$ & Homogeneous coordinates transformation of 3D point $X$ using the perspective projection function \\
%         $n$ & Number of fiducial markers \\
%         $\mathbf{z}$ & Set of YoloTag detections to $m$ observed landmarks, where $\mathbf{z} = \{z_1, z_2, \ldots, z_m\}$ \\
%         $\mathbf{x}$ & UAV pose, where $\mathbf{x} = \{x, y, z, \theta\}$ \\
%         $\mathbf{x}^*$ & Estimated UAV pose \\
%         $p(\mathbf{x} | L, \mathbf{z})$ & Maximum likelihood estimation of UAV pose given detected landmarks \\
%         $p(z | \mathbf{x}, L)$ & Landmark measurement model \\
%         $h(\mathbf{x}, l_i)$ & True range and bearing from pose $\mathbf{x}$ to landmark $l_i$ \\
%         $w$ & Noise in landmark measurement \\
%         Extended Kalman Filter & Filtering algorithm for pose estimation using landmarks \\
%         Particle filter & Filtering algorithm for pose estimation using landmarks, particularly suited for non-linear and non-Gaussian systems \\
%         \hline
%     \end{tabular}
%     \caption{Notation Table}
%     \label{tab:notations}
% \end{table}




==> sect/premable.tex <==

\usepackage{etoolbox}
\makeatletter 
\let\NAT@parse\undefined
\makeatother
\usepackage[numbers]{natbib} 

\usepackage{multirow}
\usepackage[bookmarks=true, colorlinks=false,
    linkcolor=black,
    filecolor=magenta,      
    urlcolor=cyan]{hyperref}

\usepackage{graphicx} % For importing graphics 
\usepackage{amsfonts,amssymb,amsmath} 
\usepackage{config/psfig} 
\usepackage{graphics} 
\usepackage{epsfig} 
\usepackage[all]{xy}  
% \usepackage[linesnumbered, ruled,vlined]{algorithm2e}
\usepackage{algorithm}
\usepackage{algpseudocode}
\newcommand\mycommfont[1]{\footnotesize\rmfamily{#1}}
% \SetCommentSty{mycommfont}
\usepackage[labelfont=small,textfont={small}]{caption}
\usepackage{subcaption}
\usepackage{epstopdf} 
\usepackage{balance}
\usepackage{color}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}
\usepackage{amsmath}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\usepackage[table,xcdraw]{xcolor}
\usepackage{pgf}
\usepackage{adjustbox}

==> sect/related_work.tex <==



\subsection{Vision-based localization}

Vision-based localization refers to estimating the location and pose of an agent (e.g. robot, vehicle) using cameras as the primary sensors. Two main approaches exist \textemdash Relative Visual Localization (RVL) and Absolute Visual Localization (AVL)~\cite{couturier2021review}.
RVL methods like Visual Odometry (VO) and Visual SLAM (VSLAM) incrementally estimate an agent's ego-motion as well as map previously unexplored environments by tracking visual features across frames~\cite{scaramuzza2011visual}. VO suffers from drift over long durations while VSLAM creates globally consistent maps to minimize drift~\cite{7946260}. However, VSLAM can still experience drift, inconsistencies, and computational complexity issues, especially in challenging environments or resource-constrained systems.  Prominent techniques include optical flow-based VO~\cite{Zhu2018EVFlowNetSO}, ORB-SLAM~\cite{7219438}, OKVIS~\cite{article} and VINS-Mono~\cite{8421746}. Multi-sensor fusion with IMU, wheel encoder data is used to improve robustness and address scale ambiguity in monocular VO~\cite{article1}. On the other hand, the
AVL method relies on matching ground imagery to geo-referenced offline maps to achieve drift-free, global localization~\cite{couturier2021review}. Approaches use orthorectified satellite maps~\cite{4215064}, registration of UAV images to satellite imagery~\cite{Chiu2013RobustVN}, and detection of landmarks like road markings, intersections to match against map data~\cite{Gruyer2014MapaidedLW}. A key benefit of AVL is bounded localization error due to independence from sequential estimates.

\subsection{Fiducial Marker-based Localization}

Fiducial markers have become ubiquitous for enabling precise camera tracking and localization in augmented reality (AR), virtual reality (VR), and robotics systems. The design and robust detection of visual tags has seen significant research over the past two decades.
Early square barcode-style markers like ARToolkit~\cite{kato1999} provided a foundation for many later systems. AprilTag~\cite{Olson2011AprilTagAR} offered reliable detection under real-world challenges like low resolution, occlusion, uneven lighting, and perspective distortion through its simplified binary block layout and efficient line-based detection algorithm. However, AprilTag had limitations in terms of computational efficiency and scalability to large marker sets. AprilTag 2~\cite{7759617} further improved detection speed, accuracy, and false positive rejection, but still struggled with highly distorted or blurred markers.
ChromaTag~\cite{DeGol2017ChromaTagAC} incorporated color information into the tag design with separate channels for detection, localization, and encoding. This allowed false positives to be reduced by focusing on the red-green color gradient for initial detection. DeepChArUco~\cite{Hu2018DeepCD} combined chessboard-like arrays with ArUco markers and used convolutional neural networks for robust point detection.

Recent focus has been on improving marker robustness against distortions. DeepFormableTag~\cite{Yaldiz_2021} leveraged generative adversarial networks to enable recognition under severe perspective skewing, stretching, and deformation. This was achieved by training the system with simulated deformations. However, it requires large amounts of training data and extensive computational resources. LiDARTag~\cite{Huang_2021} introduced the novel use of LiDAR point clouds for estimating 3D marker pose by fitting known marker geometry to the points. However, it struggles with low-resolution LiDAR scans and partial occlusion of the markers.

Other novel sensing modalities like U-Star~\cite{inproceedings} developed underwater signage tags to enable navigation and wayfinding. However, U-Star struggles with turbulence and variations in water clarity, resulting in distorted and degraded tag images that are difficult to accurately recognize. E2E Marker~\cite{peace2021e2etag} applied machine learning for both generating and detecting markers in an end-to-end learned system. This allowed data-driven training for robustness against real-world variations. However, E2E Marker requires large amounts of training data which can be expensive and time-consuming to collect and annotate. Additionally, its blackbox nature reduces interpretability and debuggability compared to traditional vision-based approaches.

On the detection algorithm side, techniques like quad-tree based search used in ARTag~\cite{1467495}, parallelized detection~\cite{GarridoJurado2014AutomaticGA}, and image pyramid analysis in RUNE-Tag~\cite{5995544} have improved processing efficiency and speed. However, these approaches can still struggle with small, dense marker sets and low-power devices. Flexible deep learning frameworks like DeepTag~\cite{9773975} demonstrated the ability to incorporate various existing marker systems within a common pipeline based on ROI detection and keypoint localization. However, DeepTag requires large amounts of training data including different augmentations and distortions which is expensive to collect and annotate. It is also still computationally expensive compared to traditional vision techniques.
Overall, fiducial marker systems continue to advance with innovations in design, sensing modalities, and algorithms to meet the accuracy, speed, and robustness demands of emerging AR/VR and robotics applications. The evolution of markers is driving progress in camera tracking, on-device spatial awareness, and scene understanding.
\subsection{Autonomous Navigation Utilizing Fiducial Markers}
% Fiducial markers, which are easily detectable artificial visual markers with a known geometry, can serve as useful landmarks to enable UAV navigation and state estimation. Similar to the fiducial-based approach for ground robots in ~\cite{s23063128}, aerial drones can also leverage detectable visual markers to enable onboard state estimation for navigation without relying on external positioning systems.
UAVs can leverage fiducial markers for navigation and state estimation purposes. These fiducial markers are artificial visual markers with a known geometric shape, making them easily detectable. Similar to ground robots that utilize fiducial markers for localization and mapping~\cite{s23063128}, aerial drones can also take advantage of these visual landmarks. By detecting and tracking fiducial markers, UAVs can estimate their position and orientation without relying on external positioning systems, enabling robust onboard state estimation for navigation. Distinct fiducial tags fixed at known locations provide detectable landmarks that camera-equipped UAVs can recognize during flight to help constrain and correct the vehicle's position and orientation estimates~\cite{Amiri2022}. However, limitations include the need to physically install the fiducial markers throughout the environment which may be infeasible or obstructed at times. The authors demonstrated a machine learning model capable of precise localization using the relative posing of multiple recognized markers. For UAVs operating autonomously in indoor industrial spaces like warehouses for inspection tasks, networks of visual markers potentially mounted on infrastructure at variable altitudes could similarly be detected by drones from typical flight elevations to enable robust vision-based self-localization when satellite navigation is unavailable. However, lighting conditions and limited visual sensors on UAV platforms can restrict reliable marker identification compared to the factors affecting fiducial recognition using ground robots.



==> sect/related_work_brief.tex <==
In this section, we explore the key related work in vision-based localization methods,
the evolution of fiducial marker designs and algorithms for robust detection,
and the use of fiducial markers for enabling autonomous navigation in ground and aerial vehicles.

\subsection{Vision-based Localization}
Vision-based localization involves estimating the location and orientation of a robot using cameras as primary sensors.
Two main approaches are Relative Visual Localization (RVL) and Absolute Visual Localization (AVL)~\cite{couturier2021review}.
RVL techniques like Visual Odometry (VO)~\cite{scaramuzza2011visual,Zhu2018EVFlowNetSO,article1} and Visual Simultaneous Localization and Mapping (VSLAM)~\cite{7946260,7219438,article,8421746} incrementally estimate a robot's ego-motion and map unexplored environments by tracking visual features across frames.
However, they suffer from drift over long durations. Absolute Visual Localization (AVL)~\cite{4215064,Chiu2013RobustVN,Gruyer2014MapaidedLW} aims to achieve drift-free global localization by matching imagery to geo-referenced maps, but can have limited precision.

\subsection{Fiducial Marker-based Localization}
Fiducial markers have enabled precise camera tracking for augmented/virtual reality and robotics.
Designs like ARToolKit~\cite{kato1999}, AprilTag~\cite{Olson2011AprilTagAR,7759617} and ChromaTag~\cite{DeGol2017ChromaTagAC} provide robust detection under challenges like occlusion and lighting variations.
Recent work has focused on improving marker robustness to distortions through techniques like deep neural networks~\cite{Hu2018DeepCD,Yaldiz_2021,9773975} and alternate sensing modalities like LiDAR~\cite{Huang_2021}.
Novel applications include underwater markers for navigation~\cite{inproceedings} and end-to-end learned marker generation and detection~\cite{peace2021e2etag}.
Algorithmic improvements~\cite{1467495,GarridoJurado2014AutomaticGA,5995544} have also enhanced detection efficiency and scalability.
However, exiting fiducial marker-based localization still face limitations in detection speed, accuracy, and false positive rejection, particularly under challenging conditions like low resolution, occlusion, uneven lighting, and perspective distortion.

\subsection{Autonomous Navigation with Fiducial Markers}
Ground robots~\cite{s23063128} and unmanned aerial vehicles (UAVs)~\cite{Amiri2022} can leverage fiducial markers as visual landmarks for localization and mapping.
By detecting markers at known locations, they can estimate their pose without external positioning systems.
However, practical limitations exist like marker installation requirements and sensor constraints on UAVs.



==> sect/system.tex <==
% We develop an integrated system utilizing both computer vision and inertial measurements for state estimation and path planning. Specifically, the vision-based perception module initially forms an approximate maximum a posteriori (MAP) state estimate $\hat{x}$ of the platform's pose and velocity through recognition of visual environmental landmarks:
% Fig.~\ref{fig:pipeline} illustrates our UAV navigation pipeline.

% \begin{equation}
% \hat{x} = \argmax P(x | z)
% \end{equation}

% A linear controller subsequently generates appropriate thrust and attitude commands u to guide the aircraft along the desired trajectory:  
% \begin{equation}
% u = f(\hat{x})
% \end{equation}
% Concurrently, the onboard inertial measurement unit provides supplementary sensed data $\tilde{z}$ based on IMU modalities like gyroscopes and accelerometers. By reconciling these proprioceptive measurements against known coordinates L of recognized visual markers via an extended Kalman filter, the sensor fusion YOLOtag module refines pose estimates into an updated state z:
% \begin{equation}
% z = h(\tilde{z}, L) 
% \end{equation}
% Forming a closed-loop feedback system, this improved estimate serves to calibrate future vision-based state predictions amidst navigational disturbances. Overall, this cooperative visual-inertial pipeline structure aids robust and accurate state estimation and control authority needed for consistent UAV path following and disturbance rejection performance.

\begin{figure}[ht]
    \centering
    % \includegraphics[width=.4\textwidth]{figs/navigation Pipeline.pdf}
    \includegraphics[width=.4\textwidth]{figs/system_overview.pdf}
    \caption{In this figure, an integrated system for robust autonomous Unmanned Aerial Vehicle (UAV) navigation is shown, consisting of a continuous feedback loop between four key components: the Fiducial Marker Detector, which utilizes camera images ($I_t$) and Computer Vision algorithms to estimate the position and orientation ($\mathbf{x}_t$) of the markers; the Trajectory Planner, which takes in the estimated marker states and predefined waypoints ($\rho$) to generate intermediate goal points ($g_t$) along the intended route; the Controller, which calculates control inputs ($u_t$) to steer the UAV towards each successive goal point; and the UAV itself, which upon arriving at goal points, captures new images to re-estimate marker state. This closed-loop integration between Fiducial Marker detection, Trajectory Planning, Controller, and the UAV enables precise autonomous flight along predefined paths.}
    
    \label{fig:pipeline}
\end{figure}

% Our integrated vision-based UAV navigation system consists of four modules: the State Estimator ($SE$), the Trajectory Planner ($TP$), the Controller ($C$), and the Perception ($P$) module.

% The Perception module contains a vision-based object detector called YoloV8 that provides 2D bounding box detections of fiducial markers in the image frame. These 2D detections are transformed to 3D world coordinates to localize the UAV using proposed YoloTag, but often contain noise and uncertainty. To refine the localization, the State Estimator fuses the raw perception output with motion estimates using a Low Pass Filter and Extended Kalman Filter to maintain bounded uncertainty in the estimated state $\hat{x}$.

% The system operates in a loop:
% \begin{enumerate}
% \item Given estimated state $\hat{x}$ from $SE$, $TP$ computes an intermediate goal point based on mission requirements.
% \item $C$ sends control inputs $u$ to track the goal from $TP$.
% \item Upon arriving at the new location, $P$ captures images, runs YoloTag to get observation $z$, and sends $z$ to $SE$.
% \item $SE$ fuses $z$ with motion estimates to update the state estimate $\hat{x}$.
% \end{enumerate}
% This loop repeats as the UAV executes its predefined path, with $SE$ continually refining the state estimate based on perceptions $z$ and control inputs $u$.
% \todo[inline]{refer sections inside the text, draw new diagram}
% Our integrated system consists of four main components \textemdash State Estimator, Perception, Trajectory Planner, and Controller, that work in a loop to enable autonomous navigation of UAVs.
% The \textit{State Estimator (SE)} maintains an estimate of the UAV's $d$-dimensional state, including its position, orientation, and their derivatives. It starts with an initial state estimate and refines it over time by fusing sensor measurements and motion estimates. The SE uses filtering techniques like a Low Pass Filter and Extended Kalman Filter to maintain bounded uncertainty in the estimated state despite noise.
% The \textit{Perception (P)} module uses a lightweight state-of-the-art object detector called YoloV8 to detect fiducial markers (visual tags) in images captured by the UAV's camera. Then our proposed YoloTag transforms the 2D image detections to 3D world coordinates to localize the UAV. This processed visual information provides an observation measurement to the State Estimator.
% Given the current state estimate from the SE, the \textit{Trajectory Planner (TP)} computes an optimal trajectory for an input path by generating intermediate goal points for the UAV to navigate along the desired trajectory. The goals account for the current position and mission requirements.
% The \textit{Controller (C)} tracks these goal points by computing and sending control inputs to the UAV. This enables the UAV to fly towards each goal point.

% % \todo[inline]{introduce waypoints as input to Tp}
% Formally, the loop operates as follows: SE provides the current state estimate $\hat{x}_t$ at time $t$ to TP, which computes the next goal point $g_t$ using predefined waypoints as an input. C generates control inputs $u_t$ to navigate the UAV towards this goal  $g_t$. Upon reaching the new location, P captures images $I_t$, detects markers using YoloV8, and provides the observation $z_t$ to SE utilizing YoloTag. Finally, SE fuses the observation $z_t$ with motion estimates $u_t$ to update the state estimate. This process repeats continuously as new visual observations are made, allowing the UAV to autonomously navigate while keeping its state estimate updated.
% As depicted in ~\ref{fig:pipeline},Our integrated system enables autonomous navigation of UAVs through a continuous loop involving four key components: the Fiducial Marker Detector, Trajectory Planner, Controller, and the UAV itself.

% The \textit{Fiducial Marker Detector} captures images using the UAV's on-board camera and processes them to detect fiducial markers (visual tags) using the state-of-the-art YoloV8 object detector. Our proposed YoloTag algorithm then transforms the 2D image detections to 3D world coordinates to localize the UAV. Additionally, the EPnP algorithm is used to estimate the pose of the detected markers. To maintain bounded uncertainty in the estimated state despite noise and obtain a smoother trajectory, the Fiducial Marker Detector employs a Butterworth filter on the pose estimations. These filtered marker pose estimations, denoted $\mathbf{x}_t$ at time $t$, provide observation measurements to the Trajectory Planner.

% Given the marker detections from the Fiducial Marker Detector and predefined waypoints $\rho$, the \textit{Trajectory Planner} computes an optimal trajectory by generating intermediate goal points $g_t$ for the UAV to navigate along the desired path. The goals account for both the current position as well as overall mission requirements.

% The \textit{Controller} tracks these goal points by computing and sending control inputs $u_t$ to the UAV, enabling it to fly towards each goal point $g_t$ in succession.

% Formally, this autonomous navigation loop operates as follows: The Fiducial Marker Detector provides the detected marker estimations $\mathbf{x}_t$ at time $t$ to the Trajectory Planner, which computes the next goal point $g_t$ using the predefined waypoints. The Controller then generates control inputs $u_t$ to navigate the UAV towards $g_t$. Upon reaching the new location, the Fiducial Marker Detector captures images $I_t$, detects fiducial markers using YoloV8, and updates the marker estimation $\mathbf{x}_t$ using Butterworth Filter and EPnP. This full process repeats continuously with each new visual observation, enabling precise autonomous navigation.



As shown in Figure ~\ref{fig:pipeline}, the integrated system enables autonomous navigation of UAVs through a continuous feedback loop between four key modules: the Fiducial Marker Detector, Trajectory Planner, Controller, and the UAV itself.

The \textit{Fiducial Marker Detector} captures images using the UAV's on-board camera and processes them to detect fiducial markers using computer vision algorithms. 2D image detections are transformed to 3D world coordinates to localize the UAV using camera calibration parameters. Additionally, the pose of the detected markers is estimated. These marker pose estimations, denoted $\mathbf{x}_t$ at time $t$, provide observation measurements to the Trajectory Planner.  

Given the marker detections from the Fiducial Marker Detector and predefined waypoints $\rho$, the \textit{Trajectory Planner} computes a desired trajectory by generating intermediate goal points $g_t$ for the UAV to navigate along the desired path. The goals account for both the current position as well as overall mission requirements.
The \textit{Controller} makes progress toward these goal points by computing and sending control inputs $u_t$ to the UAV, enabling it to fly towards each goal point $g_t$ in succession.

Formally, the autonomous navigation loop in~Fig.\ref{fig:pipeline} operates as follows: The Fiducial Marker Detector provides the detected marker estimations $\mathbf{x}_t$ at time $t$ to the Trajectory Planner, which computes the next goal point $g_t$ using the predefined waypoints. The Controller then generates control inputs $u_t$ to navigate the UAV towards $g_t$. Upon reaching the new location, the Fiducial Marker Detector captures images $I_t$, detects fiducial markers, and updates the marker estimation $\mathbf{x}_t$. This full process repeats continuously with each new visual observation, enabling precise autonomous navigation.
